QCD and the Hadronic Final State in Deep Inelastic Scattering at HERA

The measurements of the hadronic final state in deep inelastic scattering at HERA are reviewed and discussed in the context of QCD. Covered are the general event properties in terms of energy flows, charged particle production, and charm and strangeness production. Quark fragmentation properties are studied in the Breit frame. Event shape measurements allow "power corrections" to be applied and the strong coupling alpha_s to be extracted. Other alpha_s measurements are based on dijet rates. Jet rates as well as charm production have been used to determine the gluon density in the proton. Indications have been found in the hadronic final state for unconventional, non-DGLAP evolution at small x, which could be explained with BFKL evolution. Signatures for QCD instanton effects are discussed and first search results are presented.

==> outline.tex <==
%auto-ignore

Throughout (unless stated otherwise),
the data shown have been corrected for detector effects
and QED radiation, and the errors comprise statistical
ans systematic errors added in quadrature.

